On the Parameterized Complexity of Multiway Near-Separator

We study a new graph separation problem called Multiway Near-Separator. Given an undirected graph $G$, integer $k$, and terminal set $T \subseteq V(G)$, it asks whether there is a vertex set $S \subseteq V(G) \setminus T$ of size at most $k$ such that in graph $G-S$, no pair of distinct terminals can be connected by two pairwise internally vertex-disjoint paths. Hence each terminal pair can be separated in $G-S$ by removing at most one vertex. The problem is therefore a generalization of (Node) Multiway Cut, which asks for a vertex set for which each terminal is in a different component of $G-S$. We develop a fixed-parameter tractable algorithm for Multiway Near-Separator running in time $2^{O(k \log k)} * n^{O(1)}$. Our algorithm is based on a new pushing lemma for solutions with respect to important separators, along with two problem-specific ingredients. The first is a polynomial-time subroutine to reduce the number of terminals in the instance to a polynomial in the solution size $k$ plus the size of a given suboptimal solution. The second is a polynomial-time algorithm that, given a graph $G$ and terminal set $T \subseteq V(G)$ along with a single vertex $x \in V(G)$ that forms a multiway near-separator, computes a 14-approximation for the problem of finding a multiway near-separator not containing $x$.

==> 55 <==
%PDF-1.4
%âãÏÓ
1 0 obj
   << 
      /Title ()
      /Author ()
      /Subject ()
      /Keywords ()
      /Creator (yExport 1.5)
      /Producer (org.freehep.graphicsio.pdf.YPDFGraphics2D 1.5)
      /CreationDate (D:20230209053555+01'00')
      /ModDate (D:20230209053555+01'00')
      /Trapped /False
   >>
endobj
2 0 obj
   << 
      /Type /Catalog
      /Pages 3 0 R
      /ViewerPreferences 4 0 R
      /OpenAction [5 0 R /Fit]
   >>
endobj
4 0 obj
   << 
      /FitWindow true
      /CenterWindow false
   >>
endobj
5 0 obj
   << 
      /Parent 3 0 R
      /Type /Page
      /Contents 6 0 R
   >>
endobj
6 0 obj
   << 
      /Length 7 0 R
      /Filter [/ASCII85Decode /FlateDecode]
   >>
stream
Gb"/L]8g^@DJ%a$d4`jXh(R_T"q3ING&ZG,"*746D2`*/^V9O6U*Wk7^T09<.L1ZW-bVr$;A+nN.#ObY
-.'F$i;S*l=0/7HJ)3E)hZ!,kJ,&\;B>,AIX-Jt2qW:pchu<WKf=1c&56(8iY5e7bs#[spmJl(Je3F!%
Da2/>m@W:q:[fHWeDe7@&(YkRS(k[7b2u`J,+Gnar*)nqe]25Vk88ec_'[Ll^5P^V5Jg!`+3Nq;\UD09
E=!TBC4Kdl0p6I*KB2K>s6"mu7m?>#gMZok^VZi;-iOX!pd[;mL"O8=NVA\.,prI#%$4u1U^.hk5e3+I
D62bQ-5@Kh<,@0Ji[9-qlXaZ1J3N*g:Bs1EJld+r9T,JCg7[a9#a`[*bV$j@]N(jucqB!*!.&AK,-VP-
44jL.<hSs]0D#@28g=,`Imfe*'^dp=rqfoOE*5Y:\<jJd\<`eu5J^L4[9k]C67qCP>\\+J#.P_)(,%C8
CPCgg^ducLoq0[J-V1K9b8>R."`Q:0qUEsESo9-Jne;D%gV@/en98Nk7,ruMQXbOri#(A[+<rWR,-2CT
Ohqh!)W6S[dPemF]?G,B[jlVCi)X(b>QELY2h6lYAp928rd,&mD9t#Q[D>>:3\9WFs%f4LrtOn'E).JN
W#?=.eWjZcU;k5eJEm5LjYDIr(*qc;7WS('s,7/R.`$'Q`-dg"^i@K<!7qB6jru,I#$<,u9CNf.4EL44
r=[lc(VhrE%A3fn``q.$Gft]H!M32Prn%4k02F('#ib-QbSOHi!Npr_J1lG587B!IX&QP;E,!ZW^nnl*
^cJR`>lW-A4oZ5aNH!2`qp^qGRs$5LN0qMi1I.Ltd%n'9ndY(&g[dE74B6ti`R)pentg('e"m6N>SeO3
.QFcALIo2\(<OZ2Hq"36S3:q^QW1BoY(1#407]#&S2psgNRs]#@+PCV8\WDsJ</c'KWu9t*oL(("'bi\
!&oFg87B!IX&O9OE,ErV^pV!JYW=?%I/d!64oZ5aX`.&Uq`2(-+Qf6=jhaBC=pmQG!3Q]kBm3X6[$F:t
!>`f!^]$#-GbtU6`*-;WAf_NnXHb9Y#.Q9NU^nEj78!+[YXm')i):Qh"<F9uSAr\E'+<anM%<sPOaI6J
a]!<Ng]j@\rlEEl9p#M0VFUgQ'\VY]5Z4k*js-b%gb--S;e428'"9kY-c%;p/#Gb]J7FIA!1hSlh4!l0
\o!=h#&R;71jBU7LR"Frs4Q_aT>J8Rm[7S"Vb<@bOkI+bGnSg2f)n;8j&Vt`6LkRn,j51':MJaDA&$BO
7qrYam1;#kW.7R2MTY4l!.:G)`K"(A<X@Z`=9Zl:;NDG7Fr^oTo-[90FV3]f"Y]4C0e0j<ZpE:Q5[Q2G
Z\r;pDq/P6oh0oO_!U:h0*:IDYk.fXH0kP[gfra/W4?GD'H.`/A3JCH_d5'KFSbCs<(6oadUmj@`0+i$
LG$@[Hc\-&.t,/)EJ`1f/RRCkD'j="b@Hem<]F52.]o#=.G"YebB99Bb3K/D2o9?1<r@?o[M[s!VG/q`
d9#:Ng\8#b49(Q30%i%'2O$kR<fb6jA\e^]4%;,YSm6r%eR>"aKHOAQ#3oaRq_/4(`oGdURVcs/<mcj,
"_`Mu@igOgYq^DNG2TJ`/`ImA)Pd@N5<%4#XM`3+p]#';rDU3b_Ymuhoqp4^g`PJd/reErBo=ad-1b#H
!1N0tNM?t*"H@hul3YeSLTt*[^<lYDI3*W/4WJZnDL`(DgS,a\q_7G=]AgH#mPiose[j?Fb_[7eP^.%j
jM([.L@%L[VU8XEplDRPQQhm$>r0-kmZ.2-+ner](Lkn=F)T(SC0,fSeEr"fW>bA3JiQ\<`iWX'n(R8_
RC@d9?80i,cWe4ZhmM\P1N*FQ]O6Jl*m`?'f+Q;a)A?o'd9rX_3(d;8!oPHl&qrhM-d*"pO!lB4>/Ub@
K-Ri-5<SVk\`7`7KSlu:UX%>.fAbt_e\:P';ch<D*t3C:b/P#DEtIqo\i=/l?[<t_]sK*u"(Z9LOPkH7
&-B.rG6"$K72hO&OJToB8q0e!@]NC[PF%.O999TEbQ5LgK45p-bZ0Np\Q=^2+nK9K^VI%[!uc"aU^t;U
Lu!BV@6CAI5f;0ZOMs,Iomrr7XGV.i"`odlU(`%'=UKLb4P_M:rg>PDrG9D7enK_5!3&SGdc.47^2l[Y
R[+Z"R[u="CZ2Utc9$7L>QG_[C/Gen]r]PfG/HgG*Bj.<G=O;4QkM?3A,4h?,+L`5)],.j;X,K8_CG#Z
1]@Kg/RYErd53Zsk(-="3pk_uErf5MG?r_KF0FnNXkiK_;[:YIgpi3-'$Q1NPEe.BA`EkU"/I+g0\WnP
GUb2/MgBu9Xr0EKlEkX4Hoh?('&3;X%\A#LT53hK&"Yh,mcU0b]TcgLe<nrt;f%%_J9?ifkL,BN2oVqs
G7IGQq!P-YcCI1$J9FYdKBI[h7Var1p!hN55?D?$8hbHHk*ob-KZd3Oq`-?ndu^5R*H5;7YlIDe%BrAu
*p_-ci/Im<VC#_]>2f'#;j+3"rOM_f,4-$hOH0Af0OW6<L*G:]<%RP3UH#+cZ%gJW:oa]UYYtRFb>R\c
9kE&APNbZTJ>WiP6$$X2;G7tI:AYt/]OUt.J-mNUM[dX-_^bA*WU]bRO%j5PW6I?,nbNQBqQE!&%007_
.ZehqnJtAsRWcJ9_F"2-Yc9RD)o0+g"d^F1#VHAS2"W%^qK]U2FbuXmPO]94AAO?k821N*emY0UAlk`*
MMs4!8[0WnIS0M'FSN_f;Ft%SFQi>Gh;&;E<&R(/NNE2eP+/O<Aj\Mr\m<uOnD.%;SND>(!4@uT\p3Xu
NNKT-^3])0\Y"9Jl]hTok-58-3UO=rq+Y>9%$69u]%5&9,Zma!LOW[8>a49!dDNgs:H]_BGkMh:[a&^X
M`Q+N_*5?^(#M/s^YsY0Z-#]Gk!Y3.SR<9A-5Zi,kupIH0XbE<Zt@t@FIWK1L$tVE477->`.4jn;sNYY
=8Ucf=+'\jonN@C)Y7-aq*iXr'$Vj&k=Eqg,Fm)LW+hs?2i5$==odtni3r?ai\@qj^fpNQ7j"([=*2L'
nC5?qa2enopC-4^6<ubK\j"a"%Gs9j]AX6ZajRTs3q5W+V'P^%2L55P+6ns]rEG/?+5sM$.i25_o*$^r
G]Ur*KB[3dT%jI\HpJW_:$KH;:Yg6_]MB2kH?5%VHLArmA@3AjHKse+5=^K891$tOTk$(=ng>>@4bCrU
'AKWRZ$Ut0pXFWScC]HE@/'Z=G3_q?hOdn5FnOO^UI242TuV<>;F@6kn=,(nS2V'pZ5tZKOTEtl'/O?C
?2gLa'l+k]==W<F(;>%YZ?,3T'd+P>UCNmmneYHrL/4C%H1'#+U">IS"$5LKB]%6<Kl?QZU]ks'#q<[d
8F(?M,W$4IqCq_7hSN&a4a6>l\H9.!8f^%g6UFtgiOc#UT)4^nkbTQs$lqt9k+olpg;d1J8Ok6h-QT1t
P7F'ENOmu:F=_t7dAV]\^*I6s)a8W6m(#>p/UJoQ4[Y"_rPnZL@5/ZcD8%Er%qZDC_&aAegfe([jJgVR
rUXk,biVjhlF@uPUXj>Xi2M@lrZn!0V'P]C%fM.&RFY;I/dNJa]Y=pVF2n@;E-I7NdYk9K_2>mQe,S-Q
0:ocAh"c!p'EhkslJT4.`Ed7dGYaknpN&LC0-uuA"/M`hHo*1QGQSAEP>G,G`X2[`^'e!>PX%%mRc:BG
Xugk,>QG-;[>[.@a'FTS8$;g+Hg9V$T;s\"-(#@,U7mUgIQ!r-L??S[E8:NC!(QMgTHpFrp%',Ik*X?f
dW*19iqgsP"rN]\A29lT;\$Tall<6-j<(#_;_EIfe7IggT.>FmA6)s/:7cf9gpQj0pXIl;5P^Xm-,H)i
`l`@PapEjX?Q5Z\&eQK8F]7^Ud21c*N9)8(;cXL#iB;>;\b"tc89,\YeB)c-Mn@PXpun]PkC.FglRN;(
e9/Iq&g6euf*:/k(KBb6J7MAg8QI?OO+b<:(SHKVe90s"T.;$V1qup9cTNlJ>.`aOV_4S<am8dR$0KHS
]gQ2tA<t]dpAeG/!*L*F:m,_s,<>RdHU\*5%3:M>$'WNSb\-td;5.O>eX0<jV"163+_/QY7Q0rB+$Fc%
\T>iu!Wjm-;.n3<+5E^dKtj>TgeSD#IjMq$3D8BN>hT=e!7EaC-AAlhNp$Sb>16t7a@^X64a#YmoB-IB
Xr2BUgm;EMG/H77h)tFq'C<Js@*[8h+^7$qR@JbD!JXj[)mV2O$-]Ptff2TdSa3Sd2#R!qF6B^/HNn#N
dk'eF\YmDPCL;<^4ZrI[2<L_<F6:%to4GhC@-Rs+*WWK/'VH`/!(M"s0DC\85%2[cJ]!4:[9CB!de[rf
f&JI[nYNapQJna>Sic[@[45Ni?.@DGYD^$D^@7_?Gj\?FF0?aS5Lp[$=S#("$hfc$d'h%u!8/\a:Zl0K
Vih1p;I\*A<SE3%e7IggT.<18#t>pupESY*eo(9LWO(deXRj5/P0c#1Ekn:0\,^=(CBJ)a-QhP&e/L;?
OpdM5jWaFbL54`oVp7AJr`fH5W68hF\f?%aH#_Hi(Z&(<ci)YT`(LF!`0FX>^"F2FJuN_l>Rs(K$S[&7
(s0>'gf#,9V?CI@iulWHCMn[g!JnPl9(EF!,j.eh.1JDg#9oiV3:>?%)IU_WWX08G3%X7O;%$m1aFP:n
noE]-W-@Z"S-P'HH$Cc\nD(pt?"u<Gn^PO!5PLLk.D\,-jrTD,$'G@Ve(/pf!1IRGDX@Wl@)4[Y[!"H/
_/^--(P.Wk(-['0\9$ge%0\R(S5CZ[4WW=Sp4^8Tp=u8Tp[UohHA8PTQT9<4-W?XC_[B<:W!1lOVmq@u
ZT#oJ=>"Wm:R#Enn]=_-SND>(JA?s97\)^:]XVbE$h('ikC2j,m$A@/RHkQ(%VODsZN/F]7(^RN,k6FN
J/L8]Ua[t4/A.mP487(1"!Cl*lKl&7_-$)Z+.de'mcU`O0-uuAPBK?>F($%U8HC`6-GT@8CoBb<*^cnL
kL"kTe7n+FGs(UNCa]U4pY>X#Pb`K?7o(-gpQOd-<t``VM1Hj8h%9Ed[fm>\>.:O8(!=\PlsVbU=f4B/
WVG\Vj3Cp4:`3)OjV@(=\VIPogU1nn)f!^tjCBF;,a_M3-$f;t`1-LXL86`c#n@J/E[jML%2m>XSkTmJ
HJtd"Si_.cX"cLXdt(A?cb2"">5Q0`lJ]:G]ILUX?r$>Nk8M=:MR_U6[/l.s--B\+2;gJd&S&?WAZsSB
<uBgWFkaHV^+B>f@H@/OSNQXgE0o8preB-JJ(@?L=-CpKh`Q2"lX`en<O9T;;$Z$*!*V:2P'd?Kagp`V
;]9oC8j><\-$reU<@7sWJ2bV8$LNF$?8PEm;c-j`Q/X/4EiI-CHf/h@GOGC>!n`F;W2o)f&+3?-i`BWD
g:.%IQ2[T_F/$Yg*$`[%0F"baiRD<%Gj^/h9rBR=W!C%]lEYKocP<+);<mGW++hno(Z&)'ci)WhP$Ua7
B51,)LHZ6b.)<D04+`c"a72'6f`d"9PHa"/FkXCtk6fS=.<Y==&&DrHL6%oeHLBs2bY&9)</kT.]HDh3
q5O]i!(/l`aD&r'(eY506<e*BEfk]PYU_p,SiZ8oq/Z]r,huVRh/i%C]@Llpkc(??I^6u+P$lSe(i5R,
fEB*pfX:nbY6j0ikup1PF5T3(g:8;W_$L534W8J4gr&-S[2V;UlKGcC6XsFj0INHZUM3Op4A[m.Td50S
#+,TKP&C=H3VSke8cqlF4%p,46+!*I:CT#Rg)=:'jNF&*GUaK>)9PB+@f%II%=^aYF6Cja:bI=VF;4$!
\W;BTe?8Ss2PKh]5CN"i8qK'EQ>U.goJIL(5c9em-:c\PTSlCif6#EZA6F.Qh08:ZD[Xp63`52)\[TO`
CH$Y4eBN&!GHAQD@%O#GE*U[o0Q:jZ6SNJ+cD0W%g]XtQT"=CG2o39]RLd4Cc[@A4>.`a_Vf&+';`*Vo
"EUT_6qi*7+loJ7"%7TjSr-Y`@V"DrfEBAdDS!LVA,,Jkqp(`9UO[Z)0VOamGjaPK0"!A1%CPAJZGsP?
@*Z+^,@=`qA'[M#<?Z40lN5uGScXT+)dneuCr8K4J\QT,!<1%Ohf6Ofb)>/u0L^.Ni4O88!DEO`h@W4J
P%'Ot9dEnA,6d8\L<#Eh(3WW6GX7XqS"^AqW0ICY$6Fca\F;JR32@s*M&@uaOH^cG[1Fb?>uB&$-ij(s
j:Sph>"hlB%tMCTV^1."r'nJ%He8X$Z)-+SMaW6p"(5,E,W>][h:2Ql$R03d($#$i;\=IgFF9J.n`Ctq
VV7%nZ(/a3jHgOj\3<F(SG_aE.geJ/jZ0E@T?$*`6%5,U+3j&sa\NUYB/ATR$F9XK@#Dt"/ddn4_=5Cg
[,RuCB5r.HnC^b'S\)I/),U,,=f',,SrL>tGoOu8+*^SP4SR=6NNXRo;\(MA#(90AnZNBu&JmaPN&O9%
;/1929<'!]E_cqd0nq?Q]'S5*5;*!SJ;ZI5mc!(V[4hFe[HE#0_8Ro2jqe?e74%RDq]eMf7lUlG=4NS2
AHA6kdP\t7,D\!!=_:R:+tk_UT(iEF*OQV67uICeF-d\'Tha-XQQf5>;S1nqD+<pHri?Zbf94K:!k`M*
LYPSEPqUUk!LbR&\A?eXl#PuD&u?j(nn8oRjr1s[lFM&Wk6;23L1/TfF70?XWI<`DW'0lrB:YA%baIcr
Okk"\e$/pi6C#6,dL!/_bMAs-AsL(*_L(RZF6CjQ&9U<>lKGc#PJ,P]-@8No4SP$sk*6)@"Nr-q;aCR$
4kJ./[-5&j0!SuYgZ]>epu89rc@&p4Z_$J3FnXV^_-Le_p`!tor@+&WCC'&rND\LaCor2(JBCZ^QR^-O
3o/GVW9Z>XeQ[[BYje6qmG'o:hdkm*^nT,GHX>L8G/IBW>s7q'2<L_<F6YiY'@S503S1i2^+8-Q!TjI-
56*+Rl#69ehnYF%#cH4gUR'KH")pC'1G6K@).4`Q^Nt9R"&G3??tWR$f21iqklP*#5gKflIKgY2aV&tj
"&BAPOC[d"$ggTq8-e(!!9sW]56)PBakj(22"9,"mT;3t,7XK0/./R'?[gE/C]M$J2"YWC.;E*dS6"]V
.c2B*naPe;=Cb>L"?Y232@4dBJhMh92+t2H0c0_W?cYk)8FOn=[([nh</6qEBL/Xq3\q<[ncPPYrp*&E
%8a==d_M%^h`4nbEe&d1K_c^.<3%:R!,B*KV+*J/6nrYcBlFWu"@aEX9C/&I,7;/@,fYpT*qChbcZ?=_
?%,6<=b9P,AAq>YrsTj\no5"oiVc6$:3LdO-.,;JCgIDb'Hf?b3=/OE%.02ZTaGsFM?N9gl[c72]'eAD
\H/G%:_;pN\W;BTe@tE2e=QQZR42H60PB7^dl^EK$,uu!29cb6X_EqeWZFm$/5lrFWQWTco>jd/X_U7/
4SQ.kC[Hl&SiV5dccAHE,(_g4qi.Oa?^KpbT\&($RIr>@.Jp]XCkKRnePk(jq_j\M?@Q&Ak..sR]@=Ra
2q4Gr;s'J!&Bq-,3R`<?-#G(F'lZ;90c<5J^&a2RjQrD_B]'Q0F3\`mF\b=qCBA/)f//Sq!l*/O9(DLD
6>?5ZWTVS*o122>lVX0B'$B1DO2YC??[,@04SPaakBm`T4@*I&bO['Jc?K+de%4VkZDL97'9(nJVk-!E
9e_`!qFGqt\[TQ6P,9/S;\.4Q.2qdrJiWYG*dEf_\YQl&4[:@;jG-G[qk36XStD%"abjamnib8#?T`Ja
\UV=6J;EAU(3T0&bMo\40>+4.T)7b*p:QDn:=Y_@o:8'3Q.H/Z%tJ6kJ62aD^t6g5@%Osrh"c!pfE5MB
q0MI=ES&n\hG\(5r>@9Y]ng'f0ZWgi"J^LKJe;S^<LY>XhN+8N?ncuue7IgW%AhWU0LFSXpU7SIm0iB^
Zfh=P3T`1%F/$\41-ri->(`UCCBJN<km+?&V089qBNmhbbucDme"P<JC,NZ%*f`<G2aHNh%APPIHSOqh
]AgH#mPioseX4r$baI.9jOm',7Vf"^I7H&K;3-)\*.G'4dPP0&=NT']9V7&XT"==Eq/Z]b*ZI]lLZ9G:
6uZ'$_A?!R4SL47$[O6.4lreeC]F]1m&T_R!(ldY_%4a&?p&(#A#s5gk0r:.i1m'uU2p9]3rfjl7ZG*s
`a+LAj[ecn?]>e8htEt]D=CF9H9d77HQL%7a0c>&rLmmH1S7:E_bNZ5^V<S[]:SAh.Nubi:Yg3^ptPk+
@tKp`UM/\j7<:Aq"(+05n_Bb46SBaZVn@0/3O7t4O92ME&bb')JN+@U*q>s*^c+(a5<\\p\[/V/!RaK7
2@1f+6UFuR_KSf34nj$bjd-V(R6.JqcU\4G7)(V[YFAL]S;T$USh5:sV>)L#7j970iJXTd487(oYUFCp
Faf=;W?JF(],'qIe@tFo;^]oi>`F"X_48-TJohO>/:_iE;p0Jo*?U/EK#&mYapUEsolT!Z\H&^H8o5Rj
L:,@8G/JN"h/Bfq]u,.>_>N;u;\I>'2jV^LE3]@TiC#/ebFE>E$(tQRDH,PZn58&#i'4MT[E-21QU*.*
iJXTdN]TE@5f/@;a2]uYo%_^j>\c9Go$loYqm3Ba=-Co4QHem`&FjGTmsrU8(!l._T[P_Wqtm$nTsXQT
$?UTt5fQh%HqP8*pB=rH?.;nSm[nD*O@b$\,aCDGq;SQrcSqn1!NWIlIFIm;l-P>[kR#g[+sRNTHZbFe
_J-R]2#6*%qJn$=>![m+n0ohfMP"g,>UDQA$Ab97HLCF9!g$ajp\gAgH1&qe>O@1>eEN:rR4HmI$0F?S
#?B3@q9c/J%A'a,5RN;BhN4C`VSG)-O#@!=`Qu#N'I3"\Hg9n,e)pr!Zj>+l<U0"_GN3SK/"h1QG0BhX
NHm7pS>\0l(-.3&TsOeT(g=O>No^g`7U$^Fb2*2:q:YmL:L-,-&rZmT$jNJ%SpOYr[<BIF:u?:X<F]?.
0^!-Yfk_+8n7:jn!?s,/1V@@Rd$M.\k,MNf=YhYCnQ9Pt%CP@oT,U$r?DC8eHWo44Fp/RU?#I3FWA-%Q
R.K;^1L<T0CW0hm,D`Hi#IlBOmKtY2Dh(8sjtHJ)#6+1n9co^X,ip92Or-+7l&q1LT%9-X9-D!HecWq3
:F1K2a-Qk;6TqeoWToDf9"AhRbT5t>b8G6\p^.EkRK?a5=gAni<)d5bBmf<$!1Xl58m-+?LB*k4N^uc/
'!j*t^W];R4KtHmEg'Z[r#UsTRMkai-D??sheQ^sS-pejVlm`M+r?pUE0!&q8:*i?@MJ+Df:ZONf=TJ%
Q^VWL&0l'CI>KrABFi)C6\DejpITB6K`Q<?Q.WmGZ2bG5RGWeP(O5D6WfH239S/i>J0E\(i<SU@K"u";
]$LjoMYn"7f8co_q6!'3/470!*-%)E`b>j$j/Ctcr`td[#k?Ca=C2\jOTOhSMjngAPDJ>BU0o##93mrH
3i6XWVk6.GllQ7!4&`%1>(SLATH]XSc%J'nc[76XZDF*J"=_sYB`0/=M\CX\\3\b#JS%'8T2!%&Ka[$;
dk<T_"HF_!\66UcN*HG@T0lKYW?kdV5?8bCpBgo+bE-KCH$<B=Ug(CN8P7p<Ers,I*auA1eJJ.\\1lJ.
@gJ-['V!;^A1[X^gSh.-hA\6)MWb.4`f\c&N$Po>CO<7p:a,+*48e^Vf9<h\co1_B^(Bsi[ZOt6KBJs>
`&XXihC:U#=PGgM)/2\1_mGC-.e9/)G'AI6F)e]X1@B1rQDP!or(ELFm?c=:G$K6DH5C]f6%n\Pr[N-]
p^7^K#ahTonj6cP4=6g3T?51iTpDDiaM:@l$U[k2L4l*SiXfoQg4g/@r2=Z#NWBTg\ft;Sna;>M8UZ]X
Y"[*mJLIp'\BF^9HlkqTL>;9^"PE'i-^@>NWUSNhd"'6%T?PrOIPr*C&NBUT:(;G9@H(0se,4ukZk"b7
P)/SYqFRHK`ZhBT;uNM'@ULN8EnU!7/Vgk42NL@32eRVZ*_1$%Ei;8pgi)ELPcKZP:ubt=Re.9U>cG@)
\0S29jZ[fpD*cbIAA:'1V9Lu']A)niRpU1Xl<)CSQkQEf%9"e3(7[cF@a@qEQT63SgG+LqDWQC/=tGK8
YdVTl7ku+2liie&3jbGI?'R(+UqoHZa1P_1B4"fjFUk_^X''o0Va^r1Ca*a7eS%7Xlb)tj$bp_AT6g!f
Kj6N1Xr=d]8rCT0MFL7S&CddKkDLUi][QFU@jCokO2XmNb<fFo<BTUO7<??%Q=mhj]OoU5$1At*8[D_6
Da=U6/2YS7!dMLSEn%TTJ:9^NNVh'o'(d!J)%udr[CY.13CXZ2)<](X(/IO93nUjP#-\7FcTQ^pkMlWR
3uLPUZ$:Lcj5j\p<OQI:PgNGBH'<$Wkhs8r6tGa5^*pmLaR<$#\IYb^"VZ)@Atm5SCgiJh@%<?aLZEd1
3>>nYM'&P*D]#3!;c</Llu/;?39BtlQ=p(S'Pf^Hku!N(rBVHee32'>St&<$+!SK"1PlRc+7#T&R.S1s
4]"(UNfjMXF59u*d:U2M](NbQC"*>p/)YuE+'!=(3Ki^E\e1Hp3;?I.`i*o^[YW3*:s6u%oe!(u[+s7K
m*;oLN5PgVPOiN7ls4Je?RE"SMRFWN+TT&EqM@:t3,_eTC8?uJP!\^<mu?B6NRKQ7F_I0f"E7H)*BQ;E
:+&,<5.5>c,ttQQ`Up+AS!d_Kd]S;T4)A5\R&!9GOEnl.mu+48<1Cc4:R!BW$Fm]_<351DYc=g-$)5S'
X>rS`@rnptRAN\h\B^./B&?q$pWn]R<R6Ii!]d6DbhNISJ-0S#g7:VY4\ZE2]OU/#\KE:^O(!c*P!dV5
K+ilB`R4aZF38=-m+G7PgD&HPAG0[JAX;]n)/(&*?Fe.+*6I)Bi*S//n!au/4qa8Xj1Z*:j[jQ=!2BE7
:kk&RYVl6]iuoL'&LlVkjU@5pa"4hlU:lQ/7R6-6B<Q..V+.*qhWW0MSN-!K**eX3WUPhW:_Jn./o3d?
@c@d:n;#B!S^n"u5A)aiYb7.GFid*A]*70uhF\uSCq4Q$rDgF&"tY3j8LVm(#VhT[5Q!#j^;*F3T2BF?
@>rJa-6eKoC&g`.mK!nd!'jUE#%qL#XF;<D7h,)fpOEC^`g[#'Q`0AVhRUZ\mnniecQYid*0Ir>UU]oW
\4<)8@k8D7-j]n^-_?*9F*F$#P1pS`9+lrD/&`BT;"^RtaI+VP)%a_.cQ71O-!Utg`G-cQ$E1a)La:R7
lu#PQ8@msq7hZpG02()g`I36q_OFc67RkcQbONqdS&_!pGGt2pBoc's4+=I#m[B0nVAB/Ul;-4r@6E'0
m\Iu#j"%TdaH%(T!ZW\G?W4Qq8\X&!*mM5ch7@]lm2o.`RB1B!pE;uQq[@&t@+X!4*`+Yu;3?2`7(%E9
UrWTLq?-F919eYF*a*njC2?EOA?EN!ni_d!f)`+2,jl.ZZlB;R+uL8V/_WqL]@?a.!O&H>L3Ak!.-H"Q
7FZ6clDZF;Y\u6fU92&B\!Y:INN%1F")k;2H"9f&]Zn5aQ@t\XSl%Ld`-j!uTsXqRO&NC)+h]Sd=cE"S
:T@42rq1GuBCmhLjS:HMro5Y'@uH/qe/k%#@39^MUBQc?D<""EXj;Fa?kJS*%[/=PdNG,^Z@Up-d,@Q`
.5ne?r-2YIb%X\`CO;_J<>'LjAlq%&,m3cAmL/l&6=U,40'A!:Nk@T[D2B]32cI!lA+tNF,KP6b^Xu/h
fT7'EJ\(O7W+KjsLQ3$+52`m.P7gTWa`SEVRp*,7]@9sG-.Ut@!9u\07G^8$l8[J]1*bgNb/$S26g^_o
;dRLn8h@!b`]DZ]25$C_mh1IPXKoYkrGXA62K)'`/KD/u9jD#0B]dT+F+j*>gc<")""G@mGcFe*_oVh4
oaK0;rQa?g3*ae(.*+&sootZ(hkap44s(06h,;Nlr>StYU-:JK-T44I4Q*e`+$d)l\aD!nL*-9%gN).J
_C'#>o?dlB3I3r*HO?XR"!EHQ*cM:uS<Ve`lj=S3L0"_TLE$U[$]DVA5uN1p81dt82X6tWZo_$`0'T8#
I4nh*k=m=Ub3qEo3eY`q-cGD:]D-t!n]9_T")JC9+%EktO^rslmlS`#B>``b9X0f2+:lDeqi7Gq4"*;9
>+%MB7+.$TpbfCZ)Vn<",-sUt6jaGE1:^'N?O&jEK%rR;UA9>92L$+U=_a*Ii:GdH\Eh1n\gtCJW,pu4
dtgt3_1Djcb&4t9SNZ^/]FX@bO6a^h416@T=OT#Q3UK*I+GVT$L&1uO2]eE6lSR8*JcVJbZ%2>uc1i?L
fo=X>dXXj&k6"YJ^;&38U4_JpN4F7aP)Y=ECK`YM2.!VN)at:-Y2[Q(Gq/!M7Yj^sCIo&,Xs..dCYE_%
\-J=sr.#g(#J#u#_5N,/M@VXXG[Ost8K=%%Qte00g]PSW(`=Rgr^e3_O=>>D'TJeI2/g=e?OV&e#tEDQ
mtf`_LfB9CGb&6C<WlXUDa`+EHgnEdd^3shC,c\hhKIQE6;='q3GkUbii^g',:OeOZ-f#_HSZq!6nVZ%
qn%VRaB0<;fU#)7I'QVD/^rP>.?!&Z%9Y?OkR`Q&oY`^eID@oTViu?Z\suA\2Q*cJdm,;I?4&bJ`A6Hs
5oXdR?AWoj^l].QA3EZ(2MZb]9\o1&32%r;5`QKQ]SQdof:*V1W"!0hZ-1(9'Cj`:AS!\#!D0i-'9M%:
&LX9?2e)+f`:IM=(QS%=F[E,Ms8(CAp3Yg7GAe,WQ_W@X`[cI,HSo%2,^mD)[ua8E6rPpQ5eR?]c#HNt
3LhI8_1"AV98Kc@\BPOWlsJUu$uGhRq"[@Ns5uUg/`q9Bnpj`C70B:LA@L3.=[,94ia:UBK3J2>\,QZ#
[K1"~>
endstream
endobj
7 0 obj
   13044
endobj
3 0 obj
   << 
      /Parent null
      /Type /Pages
      /MediaBox [0.0000 0.0000 593.00 545.00]
      /Resources 8 0 R
      /Kids [5 0 R]
      /Count 1
   >>
endobj
9 0 obj
   [/PDF /Text /ImageC]
endobj
10 0 obj
   << 
      /S /Transparency
      /CS /DeviceRGB
      /I true
      /K false
   >>
endobj
11 0 obj
   << 
      /Alpha1
      << 
         /ca 1.0000
         /CA 1.0000
         /BM /Normal
         /AIS false
      >>
   >>
endobj
8 0 obj
   << 
      /ProcSet 9 0 R
      /ExtGState 11 0 R
   >>
endobj
xref
0 12
0000000000 65535 f 
0000000015 00000 n 
0000000315 00000 n 
0000013787 00000 n 
0000000445 00000 n 
0000000521 00000 n 
0000000609 00000 n 
0000013763 00000 n 
0000014241 00000 n 
0000013957 00000 n 
0000013996 00000 n 
0000014098 00000 n 
trailer
<< 
   /Size 12
   /Root 2 0 R
   /Info 1 0 R
>>
startxref
14314
%%EOF

